Domain-Specific Block Selection and Paired-View Pseudo-Labeling for Online Test-Time Adaptation

Test-time adaptation (TTA) aims to adapt a pre-trained model to a new test domain without access to source data after deployment. Existing approaches typically rely on self-training with pseudo-labels since ground-truth cannot be obtained from test data. Although the quality of pseudo labels is important for stable and accurate long-term adaptation, it has not been previously addressed. In this work, we propose DPLOT, a simple yet effective TTA framework that consists of two components: (1) domain-specific block selection and (2) pseudo-label generation using paired-view images. Specifically, we select blocks that involve domain-specific feature extraction and train these blocks by entropy minimization. After blocks are adjusted for current test domain, we generate pseudo-labels by averaging given test images and corresponding flipped counterparts. By simply using flip augmentation, we prevent a decrease in the quality of the pseudo-labels, which can be caused by the domain gap resulting from strong augmentation. Our experimental results demonstrate that DPLOT outperforms previous TTA methods in CIFAR10-C, CIFAR100-C, and ImageNet-C benchmarks, reducing error by up to 5.4%, 9.1%, and 2.9%, respectively. Also, we provide an extensive analysis to demonstrate effectiveness of our framework. Code is available at https://github.com/gist-ailab/domain-specific-block-selection-and-paired-view-pseudo-labeling-for-online-TTA.

==> sec/1_introduction_v1.tex <==
\section{Introduction}
\label{sec:intro}

% TTA에 대한 설명 및 백그라운드
When the training and target data originate from the same domain, deep neural networks achieve remarkable performance \cite{SimonyanZ14a, renNIPS15fasterrcnn}. However, deployed models often encounter performance degradation due to the domain shifts between the training data and target test data\cite{hendrycks2019robustness, recht2019imagenet, geirhos2018generalisation}. For example, a pre-trained image classification model may suffer this phenomenon for the given corrupted images due to sensor degradation, weather change, and many other reasons. To overcome this issue, various researchers have addressed the domain shift issue \cite{gong2021dlow, zhou2022domain, lu2022domain, hoyer2023mic}. For instance, domain generalization aims to train a model that can perform well on data from diverse domains and unsupervised domain adaptation aims to mitigate performance drop for the target domain using unlabeled target data\cite{hoyer2023mic, }. Recently, test-time adaptation (TTA), which aims to improve domain robustness during the deployment stage without access to the training data, has received attention because of its practicality and applicability \cite{wang2021tent, wang2022continual, gandelsman2022test, liu2021ttt}.

% Continual TTA에 대한 설명 및 베이스라인 소개
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.49\textwidth]{imgs/observation.pdf}
  \caption{Error rate on corrupted data on gradual setting (a) and Error rate on source test data (b) of various test-time adaptation methods based on entropy-minimization using CIFAR100-C and ResNext-29 architecture. It is demonstrated that the TENT applied on all batch normalization layers suffers from catastrophic forgetting (dark line), but the TENT applied on a first block does not suffer from catastrophic forgetting (orange line) and achieves competitive performance.}
  \label{fig:observation}
\end{figure}

% Online TTA에 대한 설명 및 예시.
% In detail, TTA leverages the test data during the deployment stage in offline or online. Offline TTA considers a scenario in which the model adapts with access to all test data\cite{wang2021tent, niu2022efficient, gandelsman2022test}, whereas online TTA considers the setting where the model predicts and adapts for the current test batch in real-time\cite{wang2022continual, dobler2023robust, colomer2023toadapt}. The challenging setting of online TTA requires the adaptation method to have the following attributes: 1)~robustness to catastrophic forgetting, 2)~robustness to error accumulation\cite{wang2022continual}. For example, Wang \etal\cite{wang2022continual} proposed stochastic restore, which restores the small part of the parameters in the network back to the pre-trained source model to reduce forgetting. Also, they use augmented-averaged predictions to provide an accurate pseudo-label for the network and reduce error accumulation. However, the entropy-based method namely TENT\cite{wang2021tent}, where the model is updated to reduce entropy for unseen test data, is an TTA method and suffers from performance degradation in the online TTA setting as shown in Figure \ref{fig:observation}. Therefore, we ask the following question: \textit{Can we stabilize the entropy minimization for life-long test-time adaptation?}

In detail, TTA leverages the test data during the deployment stage in offline or online. Offline TTA considers a scenario in which the model adapts with access to all test data\cite{wang2021tent, niu2022efficient, gandelsman2022test}, whereas online TTA considers the setting where the model predicts and adapts for the current test batch in real-time\cite{wang2022continual, dobler2023robust, colomer2023toadapt}. The challenging setting of online TTA requires the adaptation method to have the following attributes: 1)~robustness to catastrophic forgetting (i.e., preserving knowledge about source domain), 2)~robustness to error accumulation (i.e., preventing degradation from inaccurate learning objective)\cite{wang2022continual}. For example, Wang~\etal~\cite{wang2022continual} proposed stochastic restore, which restores the small part of the parameters in the network back to the pre-trained source model to reduce forgetting. Also, they use augmented-averaged predictions to provide an accurate pseudo-label for the network and reduce error accumulation.

However, the entropy-based method namely TENT\cite{wang2021tent}, where the model is updated to reduce entropy for unseen test data, suffers from performance degradation in the online TTA setting as shown in Figure \ref{fig:observation}. It is known that the entropy-minimization alone can lead to model collapse, which means the model predicts all samples to the same class\cite{niu2023towards}. To solve an issue, Niu~\etal~\cite{niu2022efficient} proposed EATA, where only reliable and non-redundant samples, which are low-entropy samples, are used for entropy minimization. Also, Niu~\etal~\cite{niu2023towards} proposed SAR, where only samples with small gradient norm are used for optimization. Even though these methods stabilize the entropy minimization for test-time adaptation, they still have performance degradation from a forgetting for life-long TTA setting, as shown in Figure \ref{fig:observation}. Thus, we ask the following question: \textit{How can we minimize the performance degradation of the entropy minimization for life-long test-time adaptation?}


% Motivation 언급 및 이에 기반한 제안 방법으로의 발전
In this work, we propose \textbf{s}elective \textbf{e}ntropy \textbf{m}inimization for \textbf{o}nline test-time adaptation (dubbed \textbf{SEMO}), which improves the two aforementioned attributes based on TENT\cite{wang2021tent}. The first component of the SEMO is selective block training to alleviate catastrophic forgetting. This is motivated by our observation on the entropy with regard to the blocks of the neural network. As depicted in Figure \ref{fig:observation}, we observed that employing entropy solely with the first block opposed to all batch normalization layers as done in \cite{wang2021tent, niu2022efficient, niu2023towards} significantly decrease the forgetting issue. The second component is the use of paired-view consistency (PC) loss along with entropy to combat error accumulation. PC loss forces the model to produce the same probability distribution as the mean teacher's. We are motivated by the insight that entropy loss alone leads to model collapse. Also, we find that paired-view prediction is more accurate than average prediction of many augmentations as in~\cite{wang2022continual}.

% Summary
We perform extensive evaluations and establish state-of-the-art performance on various online TTA benchmarks, including continual and gradual settings. Also, we provide empirical insight of how our method works. In summary, our key results and contributions are:
\begin{itemize}
    \item By analyzing the previous method TENT\cite{wang2021tent}, we motivate and propose the SEMO. SEMO alleviates the error accumulation and the catastrophic forgetting of the TENT which leads to stable TTA for online settings. 
    \item We conduct a various online TTA benchmarks including \textit{continual} and \textit{gradual} setting and show that our framework outperforms other method. For example, our method outperforms the best baseline by up to 9.3\% and 5.7\% on CIFAR10-C and CIFAR100-C gradual setting benchmarks, respectively.
    \item We provide a wide range of analysis that lead to an improved understanding of our framework. Moreover, we provide the online adaptation results on segmentation tasks, which show our method can be applicable to various tasks.
\end{itemize}
%-------------------------------------------------------------------------


==> sec/2_preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

% Test-Time Adaptation 설명
For a model $\theta$ pre-trained on the source data $(\mathcal{X}^S, \mathcal{Y}^S)$, TTA aims to improve the performance of the model during test-stage in the absence of
access to the source data. Here, an arbitrary function $g(\theta_t, \mathcal{X}^T)\rightarrow\theta_{t+1}$ adjusts the network parameters to $\theta_t$ using the given test data $\mathcal{X}^T$ at time $t$. Thus, TTA finds the function $g$ that effectively adjusts the parameters to alleviate the performance gap due to domain differences between $\mathcal{X}^S$ and $\mathcal{X}^T$. In an online setting, the prediction and adaptation should be made simultaneously for the given test batch $x_t \in \mathcal{X}^T$, where $t$ indicates the current time. Consider the function $g(\theta_t, x_t)\rightarrow \hat{y}, \theta_{t+1}$, where $\hat{y}$ and $\theta_{t+1}$ refer to the prediction for the given batch and the updated weight parameter, respectively. 


% Online setting 설명
% Since we cannot obtain the ground-truth of the test batch, the function is based on self-supervised learning such as consistency learning \cite{tarvainen2017mean, sohn2020fixmatch} or contrastive learning \cite{chen2020simple, wang2022contrastive}. For example, previous entropy-minimization method, TENT \cite{wang2021tent}, adjusts batch normalization weights \cite{ioffe2015batch} to minimize the entropy $H(\hat{y})$ of model predictions $\hat{y} = f(x^t;\theta)$, measured by Shannon entropy \cite{6773024}.






